FineGym: A Hierarchical Video Dataset for Fine-grained Action Understanding

On public benchmarks, current action recognition techniques have achieved great success. However, when used in real-world applications, e.g. sport analysis, which requires the capability of parsing an activity into phases and differentiating between subtly different actions, their performances remain far from being satisfactory. To take action recognition to a new level, we develop FineGym, a new dataset built on top of gymnastic videos. Compared to existing action recognition datasets, FineGym is distinguished in richness, quality, and diversity. In particular, it provides temporal annotations at both action and sub-action levels with a three-level semantic hierarchy. For example, a "balance beam" event will be annotated as a sequence of elementary sub-actions derived from five sets: "leap-jump-hop", "beam-turns", "flight-salto", "flight-handspring", and "dismount", where the sub-action in each set will be further annotated with finely defined class labels. This new level of granularity presents significant challenges for action recognition, e.g. how to parse the temporal structures from a coherent action, and how to distinguish between subtly different action classes. We systematically investigate representative methods on this dataset and obtain a number of interesting findings. We hope this dataset could advance research towards action understanding.

==> fig_confusion.tex <==
\begin{figure*}[]
	\centering
	\begin{subfigure}[t]{0.22\textwidth}
		\includegraphics[height=1.8in]{figures/tsn_sub21_rgb.png}
		\caption{TSN}
		\label{fig:tsn_sub21}
	\end{subfigure}
	\hspace{14pt}
	\begin{subfigure}[t]{0.22\textwidth}
		\includegraphics[height=1.8in]{figures/TRN_sub21_rgb.png}
		\caption{TRN}
		\label{fig:trn_sub21}
	\end{subfigure}%
	\hspace{14pt}
	\begin{subfigure}[t]{0.22\textwidth}
		\includegraphics[height=1.8in]{figures/I3D_sub21_imnet.png}
		\caption{I3D}
		\label{fig:tsm_sub21}
	\end{subfigure}
	\hspace{14pt}
	\begin{subfigure}[t]{0.22\textwidth}
		\includegraphics[height=1.8in]{figures/ST-GCN_sub21.png}
		\caption{ST-GCN}
		\label{fig:stgcn_sub21}
	\end{subfigure}
	\caption{Normalized confusion matrix of different methods on FX-S1 (\emph{Leap-jump-hop} in \emph{Floor Exercise}).}
	\label{fig:cm_sub21}
	\vspace{-7pt}
\end{figure*}

\begin{figure*}[]
	\centering
	\begin{subfigure}[t]{0.22\textwidth}
		\includegraphics[height=1.8in]{figures/tsn_sub41_rgb.png}
		\caption{TSN}
		\label{fig:tsn_sub41}
	\end{subfigure}
	\hspace{14pt}
	\begin{subfigure}[t]{0.22\textwidth}
		\includegraphics[height=1.8in]{figures/TRN_sub41_rgb.png}
		\caption{TRN}
		\label{fig:trn_sub41}
	\end{subfigure}%
	\hspace{14pt}
	\begin{subfigure}[t]{0.22\textwidth}
		\includegraphics[height=1.8in]{figures/I3D_sub41_imnet.png}
		\caption{I3D}
		\label{fig:tsm_sub41}
	\end{subfigure}
	\hspace{14pt}
	\begin{subfigure}[t]{0.22\textwidth}
		\includegraphics[height=1.8in]{figures/ST-GCN_sub41.png}
		\caption{ST-GCN}
		\label{fig:stgcn_sub41}
	\end{subfigure}
	\caption{Normalized confusion matrix of different methods on UB-S1 (\emph{The Circles} in \emph{Uneven Bars}).}
	\label{fig:cm_sub41}
	\vspace{-7pt}
\end{figure*}

==> fig_histogram.tex <==
\begin{figure*}[]
	\centering
	\begin{subfigure}[t]{\textwidth}
		\includegraphics[height=1.8in]{figures/histogram_gym_full.pdf}
		\caption{All classes}
		\label{fig:hist_all}
		\vspace{30pt}
	\end{subfigure}
	\begin{subfigure}[t]{\textwidth}
		\includegraphics[height=1.8in]{figures/histogram_gym_288.pdf}
		\caption{\emph{Gym288}}
		\label{fig:hist_gym288}
		\vspace{30pt}
	\end{subfigure}
	\begin{subfigure}[t]{\textwidth}
		\includegraphics[height=1.8in]{figures/histogram_gym_99.pdf}
		\caption{\emph{Gym99}}
		\label{fig:hist_gym99}
	\end{subfigure}
	\caption{Frequency of element classes in (a) \emph{FineGym} as well as its subset: (b) \emph{Gym288} and (c) \emph{Gym99}  \wrt sub-action instances.}
	\label{fig:histogram}
	\vspace{-7pt}
\end{figure*}

==> fig_overview.tex <==
 \begin{figure*}[!t]
	\centering
	\includegraphics[width=\linewidth]{figures/overview.pdf}
	\caption{\small  Overview of the annotations.   }
	\label{fig:overview}
\end{figure*}

==> tab_recog_element_all.tex <==
\begin{table}[]
	\small
	\centering
	\setlength\tabcolsep{4pt}
	\begin{tabular}{c @{\hspace{1\tabcolsep}}ccccc}
		\midrule[1pt]
		\multicolumn{2}{c}{\textbf{Model Info}}                            & \multicolumn{2}{c}{\textbf{\textit{Gym288}}}                     & \multicolumn{2}{c}{\textbf{\textit{Gym99}}}                      \\ 
		\midrule[1pt]
		\textbf{Method}                        & \multicolumn{1}{c}{\textbf{Modality}} & \textbf{Mean} & \multicolumn{1}{c}{\textbf{Top-1}} & \multicolumn{1}{c}{\textbf{Mean}} & \textbf{Top-1} \\     \bottomrule[1pt]
		\multicolumn{1}{c|}{ActionVLAD~\cite{girdhar2017actionvlad}}                  				& \multicolumn{1}{c|}{RGB}      		& 16.53        & \multicolumn{1}{c|}{60.52}      & 50.08                             & 69.53      \\ \hline
		\multicolumn{1}{c|}  {\multirow{3}{*}{TSN~\cite{wang2018temporal}} }         		 & \multicolumn{1}{c|}{RGB}      		& 26.54        & \multicolumn{1}{c|}{68.34}      & 61.40                             & 74.80      \\
		\multicolumn{1}{c|}{}            										& \multicolumn{1}{c|}{Flow}     		& 38.71        & \multicolumn{1}{c|}{78.30}      & 75.62                             & 84.72      \\
		\multicolumn{1}{c|}{}	 		  									    & \multicolumn{1}{c|}{2Stream}  	& 37.57        & \multicolumn{1}{c|}{79.86}      & 76.35                             & 86.03      \\ \hline
		\multicolumn{1}{c|}{\multirow{3}{*}{TRN~\cite{zhou2017temporalrelation}}}            		 & \multicolumn{1}{c|}{RGB}      		& 33.09        & \multicolumn{1}{c|}{73.75}      & 68.68                             & 79.08      \\
		\multicolumn{1}{c|}{}													&\multicolumn{1}{c|}{Flow}     			& 42.64        & \multicolumn{1}{c|}{79.48}      & 77.18                             & 84.99      \\
		\multicolumn{1}{c|}{}													& \multicolumn{1}{c|}{2Stream}  	& 42.85        & \multicolumn{1}{c|}{81.64}      & 79.75                             & 87.38      \\ \hline
		\multicolumn{1}{c|}{\multirow{3}{*}{TRNms~\cite{zhou2017temporalrelation}}} 	& \multicolumn{1}{c|}{RGB}      		& 32.01        & \multicolumn{1}{c|}{73.15}      & 68.77                             & 79.45      \\
		\multicolumn{1}{c|}{}													& \multicolumn{1}{c|}{Flow}     		& 43.41        & \multicolumn{1}{c|}{79.72}      & 77.56                             & 85.46      \\
		\multicolumn{1}{c|}{}													& \multicolumn{1}{c|}{2Stream}  	& 43.25        & \multicolumn{1}{c|}{81.98}      & 80.20                             & 87.77      \\ \hline
		\multicolumn{1}{c|}{\multirow{3}{*}{TSM~\cite{lin2019tsm}}}          			 & \multicolumn{1}{c|}{RGB}      		& 34.82        & \multicolumn{1}{c|}{73.51}      & 70.64                             & 80.38      \\
		\multicolumn{1}{c|}{}													& \multicolumn{1}{c|}{Flow}     		& 45.99        & \multicolumn{1}{c|}{81.56}      & 80.29                             & 87.14      \\
		\multicolumn{1}{c|}{}													& \multicolumn{1}{c|}{2Stream}  	& 46.46        & \multicolumn{1}{c|}{83.05}      & 81.24                             & 88.37      \\ \hline
		\multicolumn{1}{c|}{I3D~\cite{carreira2017quo}}         		& \multicolumn{1}{c|}{RGB}      & 27.87        & \multicolumn{1}{c|}{66.65}      & 63.21                             & 74.79      \\
		\multicolumn{1}{c|}{I3D$^{*}$~\cite{carreira2017quo}}         		& \multicolumn{1}{c|}{RGB}      & 28.19        & \multicolumn{1}{c|}{66.07}      & 64.41                             & 75.58      \\ \hline
		\multicolumn{1}{c|}{NL I3D~\cite{Wang2018non}}      	& \multicolumn{1}{c|}{RGB}      & 27.07        & \multicolumn{1}{c|}{64.00}      & 62.08                             & 73.05      \\
		\multicolumn{1}{c|}{NL I3D$^{*}$~\cite{Wang2018non}}      	  & \multicolumn{1}{c|}{RGB}      & 28.02        & \multicolumn{1}{c|}{67.00}      & 64.34                             & 75.30      \\ \hline
		\multicolumn{1}{c|}{ST-GCN~\cite{yan2018spatial}}                         			& \multicolumn{1}{c|}{Pose}     &   11.03        & \multicolumn{1}{c|}{34.03}           & 25.22                                   &36.36            \\  \toprule[1pt]
	\end{tabular}
	\caption{Action Recognition Results on \textit{Gym288} and \textit{Gym99}.}
	\label{tab:recog_element_all}
\end{table}




==> tab_recog_element_event.tex <==

\begin{table}[]
	\small
	\centering
	\setlength\tabcolsep{4pt}
	\begin{tabular}{c @{\hspace{1\tabcolsep}}ccccc}
		 \midrule[1pt]
		\multicolumn{2}{c}{\textbf{Model Info}}                            & \multicolumn{2}{c}{\textbf{VT}, \textit{6cls}}                     & \multicolumn{2}{c}{\textbf{FX}, \textit{35cls}}                      \\ 
		\midrule[1pt]
		\textbf{Method}                        & \multicolumn{1}{c}{\textbf{Modality}} & \textbf{Mean} & \multicolumn{1}{c}{\textbf{Top-1}} & \multicolumn{1}{c}{\textbf{Mean}} & \textbf{Top-1} \\   \bottomrule[1pt]
		\multicolumn{1}{c|}{Random}                  				      & \multicolumn{1}{c|}{-}      		       & 16.67        	  & \multicolumn{1}{c|}{-}              & 2.86                             & --      \\ \hline
		\multicolumn{1}{c|}{ActionVLAD~\cite{girdhar2017actionvlad}}                  				& \multicolumn{1}{c|}{RGB}      		  & 32.67        	& \multicolumn{1}{c|}{44.62}      & 56.43                             & 64.96      \\ \hline
		\multicolumn{1}{c|}  {\multirow{3}{*}{TSN~\cite{wang2018temporal}} }         		 & \multicolumn{1}{c|}{RGB}      		   & 27.84         & \multicolumn{1}{c|}{46.64}       & 58.55                             & 67.48      \\
		\multicolumn{1}{c|}{}            										& \multicolumn{1}{c|}{Flow}     		   & 23.10         & \multicolumn{1}{c|}{42.60}      & 70.72                             & 78.53      \\
		\multicolumn{1}{c|}{}	 		  									    & \multicolumn{1}{c|}{2Stream}  	    & 26.95         & \multicolumn{1}{c|}{47.53}       & 73.13                             & 81.58      \\ \hline
		\multicolumn{1}{c|}{\multirow{3}{*}{TRN~\cite{zhou2017temporalrelation}}}            		 & \multicolumn{1}{c|}{RGB}      		    &32.09        & \multicolumn{1}{c|}{47.98 }       &65.75                           & 72.01      \\
		\multicolumn{1}{c|}{}													&\multicolumn{1}{c|}{Flow}     			   & 28.85         & \multicolumn{1}{c|}{44.17}       & 74.86                             & 81.22     \\
		\multicolumn{1}{c|}{}													& \multicolumn{1}{c|}{2Stream}  	    & 31.36         & \multicolumn{1}{c|}{47.09}       & 77.54                             & 84.59      \\ \hline
		\multicolumn{1}{c|}{\multirow{3}{*}{TRNms~\cite{zhou2017temporalrelation}}} 	& \multicolumn{1}{c|}{RGB}      		  & 31.53         & \multicolumn{1}{c|}{46.64}        & 66.56                            & 73.36      \\
		\multicolumn{1}{c|}{}													& \multicolumn{1}{c|}{Flow}     		   & 29.10         & \multicolumn{1}{c|}{43.95}        & 74.84                           & 81.09      \\
		\multicolumn{1}{c|}{}													& \multicolumn{1}{c|}{2Stream}  	    & 30.10         & \multicolumn{1}{c|}{47.31}        & 78.16                             & 84.95     \\ \hline
		\multicolumn{1}{c|}{\multirow{3}{*}{TSM~\cite{lin2019tsm}}}          			 & \multicolumn{1}{c|}{RGB}      		   & 29.16        & \multicolumn{1}{c|}{42.15}        & 62.20                             & 68.78      \\
		\multicolumn{1}{c|}{}													& \multicolumn{1}{c|}{Flow}     		   & 26.18         & \multicolumn{1}{c|}{42.38}        & 76.19                             & 81.81      \\
		\multicolumn{1}{c|}{}													& \multicolumn{1}{c|}{2Stream}  		& 28.84         & \multicolumn{1}{c|}{44.84}        & 76.86                             & 83.60      \\ \hline
		\multicolumn{1}{c|}{{I3D}~\cite{carreira2017quo}}         	   & \multicolumn{1}{c|}{RGB}      			  & 31.45         & \multicolumn{1}{c|}{42.07}        & 53.72                             & 59.52      \\
		\multicolumn{1}{c|}{I3D$^{*}$~\cite{carreira2017quo}}         		 & \multicolumn{1}{c|}{RGB}      		 	& 33.35         & \multicolumn{1}{c|}{47.76}        & 52.19                             & 60.15     \\ \hline
		\multicolumn{1}{c|}{NL I3D~\cite{Wang2018non}}      	& \multicolumn{1}{c|}{RGB}      		   & 30.56          & \multicolumn{1}{c|}{45.96}        & 53.38                             & 59.79     \\
		\multicolumn{1}{c|}{NL I3D$^{*}$~\cite{WAG:2017-2020}}      	  & \multicolumn{1}{c|}{RGB}      		  	  & 30.80         & \multicolumn{1}{c|}{47.31}         & 50.89                             & 57.55      \\ \hline
		\multicolumn{1}{c|}{ST-GCN~\cite{yan2018spatial}}                         			& \multicolumn{1}{c|}{Pose}     		    &               	& \multicolumn{1}{c|}{}                  &                                      &            \\     \toprule[1pt]
	\end{tabular}
\caption{Action Recognition Results on \textit{Gym288} and \textit{Gym99}.}
\label{tab:recog_element_event}
\end{table}

==> tab_recog_element_group.tex <==

\begin{table}[]
	\small
	\centering
	\setlength\tabcolsep{4pt}
	\begin{tabular}{c @{\hspace{0.2\tabcolsep}}ccccc}
		 \toprule[1pt]
		\multicolumn{2}{c}{\textbf{Model Info}}                            & \multicolumn{2}{c}{\textbf{FX-G1}, \textit{11cls}}                     & \multicolumn{2}{c}{\textbf{UB-G1}, \textit{15cls}}                      \\ 
		\midrule[1pt]
		\textbf{Method}                        & \multicolumn{1}{c}{\textbf{modality}} & \textbf{Mean} & \multicolumn{1}{c}{\textbf{Top-1}} & \multicolumn{1}{c}{\textbf{Mean}} & \textbf{Top-1} \\     \bottomrule[1pt]
		\multicolumn{1}{c|}{Random}                  				& \multicolumn{1}{c|}{-}      		               & 9.09        	& \multicolumn{1}{c|}{-}               & 6.67                             & --      \\ \hline
		\multicolumn{1}{c|}{ActionVLAD~\cite{girdhar2017actionvlad}}                  				& \multicolumn{1}{c|}{RGB}      		  & 44.99        	& \multicolumn{1}{c|}{52.25}      & 51.85                             & 64.59      \\ \hline
		\multicolumn{1}{c|}  {\multirow{3}{*}{TSN~\cite{wang2018temporal}} }         		 & \multicolumn{1}{c|}{RGB}      		   & 31.19         & \multicolumn{1}{c|}{49.95}       & 44.84                             & 65.60      \\
		\multicolumn{1}{c|}{}            										& \multicolumn{1}{c|}{Flow}     		   & 69.59         & \multicolumn{1}{c|}{77.99}      & 65.34                            & 78.86      \\
		\multicolumn{1}{c|}{}	 		  									    & \multicolumn{1}{c|}{2Stream}  	    & 68.17        & \multicolumn{1}{c|}{78.51}       & 64.97                             & 80.01      \\ \hline
		\multicolumn{1}{c|}{\multirow{3}{*}{TRN~\cite{zhou2017temporalrelation}}}            		 & \multicolumn{1}{c|}{RGB}      		    & 58.24        & \multicolumn{1}{c|}{54.99 }       &53.56                          & 70.90      \\
		\multicolumn{1}{c|}{}													&\multicolumn{1}{c|}{Flow}     			   & 73.34         & \multicolumn{1}{c|}{79.92}       & 71.54                             & 82.46     \\
		\multicolumn{1}{c|}{}													& \multicolumn{1}{c|}{2Stream}  	    & 74.38         & \multicolumn{1}{c|}{81.85}       & 83.00                             & 70.98      \\ \hline
		\multicolumn{1}{c|}{\multirow{3}{*}{TRNms~\cite{zhou2017temporalrelation}}} 	& \multicolumn{1}{c|}{RGB}      		  & 58.50         & \multicolumn{1}{c|}{64.35}        & 55.76                             & 71.38     \\
		\multicolumn{1}{c|}{}													& \multicolumn{1}{c|}{Flow}     		   & 75.83         & \multicolumn{1}{c|}{82.63}        & 70.80                            & 82.19      \\
		\multicolumn{1}{c|}{}													& \multicolumn{1}{c|}{2Stream}  	    & 72.87         & \multicolumn{1}{c|}{80.82}        & 70.78                             &83.21      \\ \hline
		\multicolumn{1}{c|}{\multirow{3}{*}{TSM~\cite{lin2019tsm}}}          			 & \multicolumn{1}{c|}{RGB}      		   & 45.55        & \multicolumn{1}{c|}{53.28}        & 50.93                            & 66.42     \\
		\multicolumn{1}{c|}{}													& \multicolumn{1}{c|}{Flow}     		   & 75.85         & \multicolumn{1}{c|}{81.72}        & 73.05                             & 82.53     \\
		\multicolumn{1}{c|}{}													& \multicolumn{1}{c|}{2Stream}  		& 72.85         & \multicolumn{1}{c|}{79.41}        & 70.06                             & 80.83      \\ \hline
		\multicolumn{1}{c|}{I3D~\cite{carreira2017quo}}         	   & \multicolumn{1}{c|}{RGB}      			  & 33.34         & \multicolumn{1}{c|}{38.87}        & 32.20                             & 49.08      \\
		\multicolumn{1}{c|}{I3D$^{*}$~\cite{carreira2017quo}}         		 & \multicolumn{1}{c|}{RGB}      		 	& 36.12         & \multicolumn{1}{c|}{42.86}        & 31.02                             & 48.13     \\ \hline
		\multicolumn{1}{c|}{NL I3D~\cite{Wang2018non}}      	& \multicolumn{1}{c|}{RGB}      		   &31.43         & \multicolumn{1}{c|}{39.00}        & 29.32                             & 48.54     \\
		\multicolumn{1}{c|}{NL I3D$^{*}$~\cite{Wang2018non}}      	  & \multicolumn{1}{c|}{RGB}      		  	  & 35.84        & \multicolumn{1}{c|}{40.08}         & 26.91                           & 48.54      \\ \hline
		\multicolumn{1}{c|}{ST-GCN~\cite{yan2018spatial}}                         			& \multicolumn{1}{c|}{Pose}     		    &  21.64             	& \multicolumn{1}{c|}{30.76}                  &   13.66                                   & 28.14           \\   \toprule[1pt]
	\end{tabular}
\caption{Action Recognition Results on \textit{Gym288} and \textit{Gym99}.}
\label{tab:recog_element_group}
\end{table}
